Optical studies of two stripped envelope supernovae SN 2015ap (Type Ib) and SN 2016P (Type Ic)

We present the photometric and spectroscopic studies of a Type Ib SN 2015ap and a Type Ic SN 2016P. SN 2015ap is one of the bright (M$_{V}$ = $-$18.04 mag) Type Ib while SN 2016P lies at an average value among the Type Ic SNe (M$_{V}$ = $-$17.53 mag). Bolometric light curve modelling of SNe 2015ap and 2016P indicates that both the SNe are powered by $^{56}$Ni + magnetar model with $^{56}$Ni masses of 0.01 M$_{\odot}$ and 0.002 M$_{\odot}$, ejecta masses of 3.75 M$_{\odot}$ and 4.66 M$_{\odot}$, spin period P$_{0}$ of 25.8 ms and 36.5 ms and magnetic field B$_{p}$ of 28.39 $\times$ 10$^{14}$ Gauss and 35.3 $\times$ 10$^{14}$ Gauss respectively. The early spectra of SN 2015ap shows prominent lines of He with a "W" feature due to Fe complexes while other lines of Mg II, Na I and Si II are present in both SNe 2015ap and 2016P. Nebular phase [O I] profile indicates an asymmetric profile in SN 2015ap. The [O I]/[Ca II] ratio and nebular spectral modelling of SN 2015ap hints towards a progenitor mass between 12 $-$ 20 M$_{\odot}$.

==> Table6.tex <==
\begin{center}
%\begin{longtable}{|c | c | c | c | c | c | c | c|}
\begin{table*}
\smallskip
\small\addtolength{\tabcolsep}{-1pt}
\caption{{\it Swift} UVOT observations of SN 2015ap}  		  
\begin{tabular}{c c c c c c c c c c}
\hline \hline
Date           & JD            & $uvw1$              & $uvw2$                 & $uvm2$    & $U$    & $B$   & $V$  \\               
	       &               & (mag)               & (mag)                  & (mag)     & (mag)  & (mag) & (mag)      \\
\hline
09/09/2015     & 2457274.9  &  17.617 $\pm$  0.217	& 18.572 $\pm$  0.116  & 18.729  $\pm$   0.112 & 16.398  $\pm$     0.101  & 17.168  $\pm$   0.098 & 16.851  $\pm$  0.127        \\    
11/09/2015     & 2457276.3  &  16.882 $\pm$  0.115	& 17.993 $\pm$  0.232  & 18.331  $\pm$   0.294 & 15.728  $\pm$     0.075  & 16.600  $\pm$   0.073 & 16.257  $\pm$  0.084        \\
13/09/2015     & 2457278.3  &  16.576 $\pm$  0.108	& 17.930 $\pm$  0.238  & 18.106  $\pm$   0.264 & 15.350  $\pm$     0.073  & 16.125  $\pm$   0.070 & 15.823  $\pm$  0.081        \\
17/09/2015     & 2457282.9  &  16.396 $\pm$  0.124	& 17.512 $\pm$  0.222  & 17.750  $\pm$   0.247 & 15.040  $\pm$     0.068  & 15.570  $\pm$   0.065 & 15.292  $\pm$  0.089        \\
18/09/2015     & 2457284.5  &  16.864 $\pm$  0.123	& 17.947 $\pm$  0.239  & 18.442  $\pm$   0.335 & 15.174  $\pm$     0.065  & 15.635  $\pm$   0.063 & 15.341  $\pm$  0.069        \\
21/09/2015     & 2457287.9  &  17.400 $\pm$  0.152	& 18.799 $\pm$  0.159  & 18.708  $\pm$   0.234 & 15.738  $\pm$     0.074  & 15.897  $\pm$   0.062 & 15.317  $\pm$  0.063        \\ 
24/09/2015     & 2457290.0  &  17.602 $\pm$  0.170	& 18.821 $\pm$  0.197  & 18.608  $\pm$   0.134 & 16.025  $\pm$     0.079  & 16.143  $\pm$   0.064 & 15.453  $\pm$  0.064        \\
26/09/2015     & 2457292.6  &  18.427 $\pm$  0.310	& 18.821 $\pm$  0.195  & 18.728  $\pm$   0.126 & 16.657  $\pm$     0.099  & 16.487  $\pm$   0.070 & 15.658  $\pm$  0.067        \\
30/09/2015     & 2457296.6  &  18.661 $\pm$  0.256 	& 18.799 $\pm$  0.168  & 18.669  $\pm$   0.132 & 17.402  $\pm$     0.148  & 17.086  $\pm$   0.085 & 16.058  $\pm$  0.077        \\
03/10/2015     & 2457299.6  &  18.662 $\pm$  0.278	& 18.798 $\pm$  0.178  & 18.695  $\pm$   0.112 & 17.843  $\pm$     0.197  & 17.283  $\pm$   0.092 & 16.217  $\pm$  0.081        \\
06/10/2015     & 2457302.9  &  18.627 $\pm$  0.221	& 18.765 $\pm$  0.168  & 18.678  $\pm$   0.123 & 18.008  $\pm$     0.228  & 17.612  $\pm$   0.111 & 16.481  $\pm$  0.094        \\
\hline          		                    
\end{tabular}
\label{tab:swiftobservation_log_2015ap}     
%\hline
\newline
\end{table*}
%\end{longtable}
\end{center} 		


